Efficient estimation of the target population average treatment effect from multi-source data

We consider estimation of the target population average treatment effect (TATE) when outcome information is unavailable. Instead, we observe the outcome in multiple source populations and wish to combine the treatment effects therein to make inference on the TATE. In contrast to existing works that assume transportability on the conditional distribution of potential outcomes or conditional treatment-specific means, we work under a weaker form of effect transportability. Following the framework for causally interpretable meta-analysis, we assume transportability of conditional average treatment effects across multiple populations, which may hold with fewer standardization variables. Under this assumption, we derive the semiparametric efficiency bound of the TATE and characterize a class of doubly robust and asymptotically linear estimators. Within this class, an efficient estimator assigns optimal weights to observations from different data sources. Additionally, we suggest estimators of a low-dimensional summary of effect heterogeneity in the target population. We illustrate the use of the proposed estimators on a multicentre weight management clinical trial for semaglutide, a glucagon-like peptide-1 receptor agonist, on overweight or obese patients. Using outcome information from other regions, we estimate the weight loss effect of semaglutide in the United States subgroup.

==> tab/ate-res-aipw.tex <==

\begin{tabular}{llrrr}
{Cross-fitting} & {Region} & {Estimate} & {SE} & {\(95\%\)-CI}\\
\(5\)-fold & EA & \(-11.16\) & \(1.36\) & \((-13.83, -8.50)\)\\
 & EU & \(-12.37\) & \(0.94\) & \((-14.22, -10.52)\)\\
 & UK & \(-14.32\) & \(1.25\) & \((-16.78, -11.87)\)\\
 & US & \(-13.18\) & \(0.66\) & \((-14.47, -11.90)\)\\
\(2\)-fold & EA & \(-12.06\) & \(1.37\) & \((-14.76, -9.37)\)\\
 & EU & \(-12.62\) & \(0.94\) & \((-14.46, -10.77)\)\\
 & UK & \(-14.12\) & \(1.29\) & \((-16.65, -11.60)\)\\
 & US & \(-13.19\) & \(0.66\) & \((-14.48, -11.90)\)\\
None & EA & \(-11.11\) & \(1.16\) & \((-13.38, -8.84)\)\\
 & EU & \(-12.64\) & \(0.81\) & \((-14.22, -11.06)\)\\
 & UK & \(-13.91\) & \(1.08\) & \((-16.03, -11.79)\)\\
 & US & \(-13.21\) & \(0.65\) & \((-14.48, -11.94)\)\\
\end{tabular}


==> tab/seed-sim-param-3-alt-cf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3105.79\) & \(310.58\) & \(7.07\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.79\) & \(310.58\) & \(7.07\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3105.64\) & \(310.56\) & \(4.97\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.64\) & \(310.56\) & \(4.97\) & \(0.0\)\\
\end{tabular}


==> tab/seed-sim-param-3-alt-nocf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.15\) & \(310.72\) & \(6.38\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.15\) & \(310.72\) & \(6.38\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.34\) & \(310.73\) & \(4.65\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.34\) & \(310.73\) & \(4.65\) & \(0.0\)\\
\end{tabular}


==> tab/seed-sim-param-3-cf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(4.42\) & \(24.92\) & \(11.48\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(4.42\) & \(24.92\) & \(11.48\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(4.68\) & \(24.83\) & \(11.52\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.12\) & \(9.78\) & \(27.47\) & \(12.11\) & \(94.5\)\\
 & 2 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.07\) & \(-36.52\) & \(57.47\) & \(11.54\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.07\) & \(-36.52\) & \(57.47\) & \(11.54\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.07\) & \(-36.66\) & \(57.54\) & \(11.52\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.08\) & \(-30.15\) & \(51.89\) & \(11.52\) & \(92.9\)\\
 & 3 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(6.95\) & \(32.00\) & \(11.60\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(6.95\) & \(32.00\) & \(11.60\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.12\) & \(7.26\) & \(32.08\) & \(11.64\) & \(93.1\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.12\) & \(12.03\) & \(37.09\) & \(12.25\) & \(92.8\)\\
 & 4 & \(\hat\theta_{\mathrm{oracle}}\) & \(2.92\) & \(-187.99\) & \(52.06\) & \(10.67\) & \(43.6\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(2.92\) & \(-187.99\) & \(52.06\) & \(10.67\) & \(43.6\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(2.92\) & \(-185.98\) & \(52.15\) & \(10.66\) & \(44.8\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(2.93\) & \(-178.38\) & \(48.97\) & \(10.84\) & \(48.0\)\\
\(2500\) & 1 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(4.02\) & \(5.67\) & \(5.56\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(4.02\) & \(5.67\) & \(5.56\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(4.03\) & \(5.67\) & \(5.57\) & \(94.1\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(4.04\) & \(5.71\) & \(5.61\) & \(94.2\)\\
 & 2 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.10\) & \(-7.50\) & \(6.55\) & \(6.10\) & \(92.2\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.10\) & \(-7.50\) & \(6.55\) & \(6.10\) & \(92.2\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.10\) & \(-7.37\) & \(6.54\) & \(6.09\) & \(92.2\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.10\) & \(-7.33\) & \(6.58\) & \(6.11\) & \(92.5\)\\
 & 3 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(1.35\) & \(5.77\) & \(5.37\) & \(93.2\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(1.35\) & \(5.77\) & \(5.37\) & \(93.2\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(1.40\) & \(5.76\) & \(5.37\) & \(93.4\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(1.28\) & \(5.82\) & \(5.41\) & \(92.3\)\\
 & 4 & \(\hat\theta_{\mathrm{oracle}}\) & \(2.93\) & \(-176.93\) & \(18.55\) & \(5.69\) & \(12.5\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(2.93\) & \(-176.93\) & \(18.55\) & \(5.69\) & \(12.5\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(2.93\) & \(-174.42\) & \(18.31\) & \(5.68\) & \(13.2\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(2.94\) & \(-164.30\) & \(17.37\) & \(5.84\) & \(18.6\)\\
\end{tabular}


==> tab/seed-sim-param-3-nocf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.10\) & \(-11.24\) & \(22.40\) & \(7.63\) & \(91.5\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.10\) & \(-11.24\) & \(22.40\) & \(7.63\) & \(91.5\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.10\) & \(-11.02\) & \(21.93\) & \(7.62\) & \(91.6\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.10\) & \(-10.40\) & \(21.63\) & \(7.37\) & \(89.4\)\\
 & 2 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.40\) & \(290.83\) & \(1077.98\) & \(17.93\) & \(86.4\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.40\) & \(290.83\) & \(1077.98\) & \(17.93\) & \(86.4\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.40\) & \(294.57\) & \(1088.37\) & \(18.02\) & \(86.4\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.54\) & \(434.36\) & \(1552.70\) & \(21.55\) & \(82.5\)\\
 & 3 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.10\) & \(-12.27\) & \(15.63\) & \(7.24\) & \(89.9\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.10\) & \(-12.27\) & \(15.63\) & \(7.24\) & \(89.9\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.10\) & \(-12.03\) & \(15.29\) & \(7.23\) & \(89.8\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.10\) & \(-11.52\) & \(15.29\) & \(6.99\) & \(87.2\)\\
 & 4 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.23\) & \(121.24\) & \(982.54\) & \(16.43\) & \(29.8\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.23\) & \(121.24\) & \(982.54\) & \(16.43\) & \(29.8\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.24\) & \(127.23\) & \(993.94\) & \(16.54\) & \(30.9\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.38\) & \(275.36\) & \(1449.13\) & \(20.19\) & \(30.3\)\\
\(2500\) & 1 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(-1.08\) & \(5.56\) & \(5.16\) & \(92.1\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(-1.08\) & \(5.56\) & \(5.16\) & \(92.1\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(-1.07\) & \(5.56\) & \(5.16\) & \(92.3\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(-1.14\) & \(5.57\) & \(5.04\) & \(91.4\)\\
 & 2 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.08\) & \(-25.42\) & \(6.83\) & \(5.55\) & \(87.9\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.08\) & \(-25.42\) & \(6.83\) & \(5.55\) & \(87.9\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.08\) & \(-25.08\) & \(6.81\) & \(5.55\) & \(87.9\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.08\) & \(-31.26\) & \(7.01\) & \(5.32\) & \(84.9\)\\
 & 3 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(-2.55\) & \(5.73\) & \(4.99\) & \(90.6\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(-2.55\) & \(5.73\) & \(4.99\) & \(90.6\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(-2.52\) & \(5.72\) & \(5.00\) & \(90.8\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(-2.60\) & \(5.76\) & \(4.88\) & \(89.5\)\\
 & 4 & \(\hat\theta_{\mathrm{oracle}}\) & \(2.93\) & \(-181.33\) & \(18.95\) & \(5.18\) & \(6.3\)\\
 &  & \(\hat\theta_{\mathrm{overlap}}\) & \(2.93\) & \(-181.33\) & \(18.95\) & \(5.18\) & \(6.3\)\\
 &  & \(\hat\theta_{\mathrm{constant}}\) & \(2.93\) & \(-178.84\) & \(18.71\) & \(5.18\) & \(7.0\)\\
 &  & \(\hat\theta_{\mathrm{optimal}}\) & \(2.94\) & \(-168.25\) & \(17.72\) & \(5.09\) & \(9.5\)\\
\end{tabular}


==> tab/sim-param-1-alt-cf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3113.81\) & \(311.39\) & \(8.43\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.59\) & \(310.56\) & \(8.90\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3113.98\) & \(311.40\) & \(5.92\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.55\) & \(310.56\) & \(6.26\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-1-alt-nocf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3113.62\) & \(311.37\) & \(7.57\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.93\) & \(310.69\) & \(8.03\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3114.07\) & \(311.41\) & \(5.48\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.72\) & \(310.67\) & \(5.82\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-1-alt.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3113.71\) & \(311.38\) & \(8.00\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.26\) & \(310.63\) & \(8.47\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3114.02\) & \(311.41\) & \(5.70\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.13\) & \(310.61\) & \(6.04\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-2-alt-cf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.88\) & \(311.22\) & \(10.47\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.80\) & \(310.59\) & \(11.25\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.75\) & \(311.19\) & \(7.32\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.38\) & \(310.54\) & \(7.89\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-2-alt-nocf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.92\) & \(311.21\) & \(9.38\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.11\) & \(310.71\) & \(10.15\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.92\) & \(311.20\) & \(6.77\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.39\) & \(310.64\) & \(7.33\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-2-alt.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.90\) & \(311.22\) & \(9.92\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.46\) & \(310.65\) & \(10.70\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.83\) & \(311.20\) & \(7.05\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.88\) & \(310.59\) & \(7.61\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-3-alt-cf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3105.60\) & \(310.56\) & \(7.06\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3105.60\) & \(310.56\) & \(7.06\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3106.01\) & \(310.60\) & \(4.97\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.01\) & \(310.60\) & \(4.97\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-3-alt-nocf.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Weight} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.17\) & \(310.72\) & \(6.38\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.17\) & \(310.72\) & \(6.38\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.26\) & \(310.73\) & \(4.62\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.26\) & \(310.73\) & \(4.62\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-3-alt.tex <==

\begin{tabular}{rlrrrrr}
{\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3106.39\) & \(310.64\) & \(6.72\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.39\) & \(310.64\) & \(6.72\) & \(0.0\)\\
\(2500\) & \(\hat\theta^\dagger\) & \(0.00\) & \(-3106.63\) & \(310.66\) & \(4.79\) & \(0.0\)\\
 & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.63\) & \(310.66\) & \(4.79\) & \(0.0\)\\
\end{tabular}


==> tab/sim-param-3-cf-small-sample.tex <==

\begin{tabular}{llrrrr}
{Experiment} & {Estimator} & {Median} & {Bias} & {MAD} & {SE}\\
1 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(4.32\) & \(5.40\) & \(7.96\)\\
 & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(4.32\) & \(5.40\) & \(7.96\)\\
 & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(4.39\) & \(5.35\) & \(7.96\)\\
 & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(2.32\) & \(5.36\) & \(8.07\)\\
2 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.08\) & \(-26.55\) & \(6.21\) & \(8.63\)\\
 & \(\hat\theta_{\mathrm{overlap}}\) & \(3.08\) & \(-26.55\) & \(6.21\) & \(8.63\)\\
 & \(\hat\theta_{\mathrm{constant}}\) & \(3.08\) & \(-26.37\) & \(6.20\) & \(8.61\)\\
 & \(\hat\theta_{\mathrm{optimal}}\) & \(3.08\) & \(-28.52\) & \(6.13\) & \(8.80\)\\
3 & \(\hat\theta_{\mathrm{oracle}}\) & \(3.11\) & \(1.58\) & \(5.48\) & \(7.71\)\\
 & \(\hat\theta_{\mathrm{overlap}}\) & \(3.11\) & \(1.58\) & \(5.48\) & \(7.71\)\\
 & \(\hat\theta_{\mathrm{constant}}\) & \(3.11\) & \(1.63\) & \(5.41\) & \(7.71\)\\
 & \(\hat\theta_{\mathrm{optimal}}\) & \(3.11\) & \(2.41\) & \(5.50\) & \(7.82\)\\
4 & \(\hat\theta_{\mathrm{oracle}}\) & \(2.93\) & \(-176.63\) & \(5.69\) & \(8.13\)\\
 & \(\hat\theta_{\mathrm{overlap}}\) & \(2.93\) & \(-176.63\) & \(5.69\) & \(8.13\)\\
 & \(\hat\theta_{\mathrm{constant}}\) & \(2.93\) & \(-173.60\) & \(5.73\) & \(8.13\)\\
 & \(\hat\theta_{\mathrm{optimal}}\) & \(2.93\) & \(-173.08\) & \(5.71\) & \(8.41\)\\
\end{tabular}


==> tab/sim-param-alt-nocf.tex <==

\begin{tabular}{rlrrrrrr}
{\(n\)} & {Setting} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & I & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3113.62\) & \(311.37\) & \(7.57\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.93\) & \(310.69\) & \(8.03\) & \(0.0\)\\
 & II & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.92\) & \(311.21\) & \(9.38\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.11\) & \(310.71\) & \(10.15\) & \(0.0\)\\
 & III & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.17\) & \(310.72\) & \(6.38\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.17\) & \(310.72\) & \(6.38\) & \(0.0\)\\
\(2500\) & I & \(\hat\theta^\dagger\) & \(-0.01\) & \(-3114.07\) & \(311.41\) & \(5.48\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.72\) & \(310.67\) & \(5.82\) & \(0.0\)\\
 & II & \(\hat\theta^\dagger\) & \(-0.00\) & \(-3111.92\) & \(311.20\) & \(6.77\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3106.39\) & \(310.64\) & \(7.33\) & \(0.0\)\\
 & III & \(\hat\theta^\dagger\) & \(0.00\) & \(-3107.26\) & \(310.73\) & \(4.62\) & \(0.0\)\\
 &  & \(\hat\theta^\ddagger\) & \(0.00\) & \(-3107.26\) & \(310.73\) & \(4.62\) & \(0.0\)\\
\end{tabular}


==> tab/sim-pcate-1-param-1-cf.tex <==

\begin{tabular}{llrlrrrrr}
{Crossfitting} & {Setting} & {\(n\)} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(5\)-fold & 1 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(6.70\) & \(14.43\) & \(13.19\) & \(94.6\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(5.39\) & \(14.52\) & \(13.86\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(5.48\) & \(14.51\) & \(13.83\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(5.82\) & \(14.74\) & \(13.45\) & \(93.9\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.01\) & \(10.26\) & \(8.61\) & \(8.96\) & \(95.2\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.01\) & \(10.85\) & \(9.17\) & \(9.46\) & \(95.8\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.01\) & \(10.93\) & \(9.15\) & \(9.44\) & \(95.9\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(10.03\) & \(8.65\) & \(9.05\) & \(96.2\)\\
 & 2 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(8.60\) & \(18.40\) & \(16.52\) & \(94.4\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(6.94\) & \(18.32\) & \(17.69\) & \(94.3\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(7.05\) & \(18.28\) & \(17.61\) & \(94.1\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(8.75\) & \(19.38\) & \(16.91\) & \(94.3\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.01\) & \(11.76\) & \(10.80\) & \(11.25\) & \(95.3\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.01\) & \(11.82\) & \(11.72\) & \(12.13\) & \(96.3\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.01\) & \(11.92\) & \(11.68\) & \(12.08\) & \(96.1\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.01\) & \(11.75\) & \(10.85\) & \(11.38\) & \(95.5\)\\
 & 3 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.76\) & \(-232.51\) & \(756.44\) & \(27.07\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.76\) & \(-232.51\) & \(756.44\) & \(27.07\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.77\) & \(-226.90\) & \(738.80\) & \(26.71\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.80\) & \(-191.26\) & \(623.07\) & \(24.46\) & \(93.6\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(9.40\) & \(7.22\) & \(7.47\) & \(95.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(9.40\) & \(7.22\) & \(7.47\) & \(95.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(9.45\) & \(7.23\) & \(7.47\) & \(95.6\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(9.02\) & \(7.25\) & \(7.54\) & \(95.9\)\\
None & 1 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.99\) & \(-2.49\) & \(16.65\) & \(11.73\) & \(92.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.99\) & \(-1.19\) & \(17.33\) & \(12.46\) & \(92.1\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.99\) & \(-1.11\) & \(17.46\) & \(12.45\) & \(91.9\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.99\) & \(-2.29\) & \(16.32\) & \(11.24\) & \(90.8\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(6.38\) & \(8.37\) & \(8.13\) & \(94.3\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(7.09\) & \(8.92\) & \(8.57\) & \(94.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(7.15\) & \(8.90\) & \(8.55\) & \(94.6\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(6.57\) & \(8.34\) & \(7.91\) & \(93.4\)\\
 & 2 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(0.65\) & \(19.23\) & \(14.64\) & \(92.3\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(1.25\) & \(22.12\) & \(15.90\) & \(92.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(1.40\) & \(22.25\) & \(15.86\) & \(92.4\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.99\) & \(-1.72\) & \(15.98\) & \(13.92\) & \(90.9\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(7.83\) & \(10.50\) & \(10.17\) & \(94.0\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(8.27\) & \(11.38\) & \(10.94\) & \(94.2\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(8.34\) & \(11.34\) & \(10.90\) & \(94.5\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(8.46\) & \(10.48\) & \(9.89\) & \(93.2\)\\
 & 3 & \(1250\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.99\) & \(-1.38\) & \(13.96\) & \(9.92\) & \(91.7\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.99\) & \(-1.38\) & \(13.96\) & \(9.92\) & \(91.7\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.99\) & \(-1.32\) & \(14.08\) & \(9.93\) & \(91.8\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.99\) & \(-2.09\) & \(12.67\) & \(9.39\) & \(91.1\)\\
 &  & \(2500\) & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(5.74\) & \(7.01\) & \(6.79\) & \(94.1\)\\
 &  &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(5.74\) & \(7.01\) & \(6.79\) & \(94.1\)\\
 &  &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(5.78\) & \(7.01\) & \(6.79\) & \(94.2\)\\
 &  &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(5.92\) & \(6.97\) & \(6.59\) & \(93.2\)\\
\end{tabular}


==> tab/sim-pcate-1-param-1-nocf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.99\) & \(-2.49\) & \(16.65\) & \(11.73\) & \(92.5\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.99\) & \(-1.19\) & \(17.33\) & \(12.46\) & \(92.1\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.99\) & \(-1.11\) & \(17.46\) & \(12.45\) & \(91.9\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.99\) & \(-2.29\) & \(16.32\) & \(11.24\) & \(90.8\)\\
 & 2 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.99\) & \(-9.64\) & \(13.63\) & \(12.41\) & \(92.9\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.98\) & \(-12.17\) & \(14.38\) & \(12.87\) & \(92.8\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.98\) & \(-11.89\) & \(14.32\) & \(12.85\) & \(92.9\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.98\) & \(-12.50\) & \(13.97\) & \(11.92\) & \(91.0\)\\
 & 3 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.99\) & \(-6.20\) & \(17.70\) & \(12.10\) & \(92.9\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.99\) & \(-5.11\) & \(18.52\) & \(12.94\) & \(92.8\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.99\) & \(-5.01\) & \(18.60\) & \(12.92\) & \(92.6\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.99\) & \(-5.51\) & \(17.45\) & \(11.58\) & \(91.6\)\\
 & 4 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.97\) & \(-26.14\) & \(14.24\) & \(12.84\) & \(93.0\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.96\) & \(-31.30\) & \(14.96\) & \(13.31\) & \(92.4\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.96\) & \(-30.72\) & \(14.89\) & \(13.29\) & \(92.4\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.97\) & \(-29.45\) & \(14.50\) & \(12.36\) & \(91.8\)\\
\(2500\) & 1 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(6.38\) & \(8.37\) & \(8.13\) & \(94.3\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(7.09\) & \(8.92\) & \(8.57\) & \(94.5\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(7.15\) & \(8.90\) & \(8.55\) & \(94.6\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(6.57\) & \(8.34\) & \(7.91\) & \(93.4\)\\
 & 2 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(3.29\) & \(9.11\) & \(8.87\) & \(94.5\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(3.12\) & \(9.55\) & \(9.18\) & \(95.0\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(3.30\) & \(9.54\) & \(9.17\) & \(94.9\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(3.02\) & \(9.06\) & \(8.59\) & \(93.7\)\\
 & 3 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(3.00\) & \(4.78\) & \(8.52\) & \(8.31\) & \(93.5\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(3.00\) & \(5.05\) & \(9.18\) & \(8.79\) & \(94.0\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(3.00\) & \(5.10\) & \(9.15\) & \(8.77\) & \(94.1\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(3.00\) & \(4.99\) & \(8.47\) & \(8.07\) & \(92.9\)\\
 & 4 & \(\hat\beta_{1,\mathrm{oracle}}\) & \(2.98\) & \(-15.05\) & \(9.55\) & \(9.18\) & \(94.1\)\\
 &  & \(\hat\beta_{1,\mathrm{overlap}}\) & \(2.98\) & \(-18.43\) & \(10.07\) & \(9.49\) & \(94.0\)\\
 &  & \(\hat\beta_{1,\mathrm{constant}}\) & \(2.98\) & \(-17.93\) & \(10.04\) & \(9.47\) & \(94.2\)\\
 &  & \(\hat\beta_{1,\mathrm{optimal}}\) & \(2.98\) & \(-15.72\) & \(9.54\) & \(8.93\) & \(93.7\)\\
\end{tabular}


==> tab/sim-pcate-2-param-1-cf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.95\) & \(15.96\) & \(40.87\) & \(38.90\) & \(95.0\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.96\) & \(21.22\) & \(41.93\) & \(40.96\) & \(95.0\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.96\) & \(20.78\) & \(41.86\) & \(40.88\) & \(95.0\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.96\) & \(19.37\) & \(41.83\) & \(39.76\) & \(95.0\)\\
 & 2 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.95\) & \(11.89\) & \(47.43\) & \(46.82\) & \(95.2\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.95\) & \(12.71\) & \(49.73\) & \(47.83\) & \(95.7\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.95\) & \(12.33\) & \(49.42\) & \(47.70\) & \(95.7\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.95\) & \(14.53\) & \(50.17\) & \(47.82\) & \(95.9\)\\
 & 3 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.96\) & \(19.95\) & \(42.90\) & \(38.90\) & \(95.8\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.97\) & \(28.73\) & \(45.89\) & \(41.29\) & \(95.7\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.97\) & \(28.09\) & \(45.57\) & \(41.15\) & \(95.4\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.96\) & \(23.97\) & \(45.93\) & \(39.87\) & \(96.2\)\\
 & 4 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.94\) & \(3.90\) & \(47.98\) & \(46.57\) & \(95.6\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(-1.20\) & \(51.46\) & \(47.70\) & \(96.5\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(-0.62\) & \(51.03\) & \(47.56\) & \(96.5\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(4.74\) & \(51.97\) & \(47.95\) & \(96.1\)\\
\(2500\) & 1 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.94\) & \(-0.27\) & \(26.20\) & \(26.33\) & \(94.2\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(0.22\) & \(27.89\) & \(27.77\) & \(94.6\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(0.35\) & \(27.83\) & \(27.72\) & \(94.6\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(0.38\) & \(26.33\) & \(26.59\) & \(94.8\)\\
 & 2 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.94\) & \(2.72\) & \(31.21\) & \(32.05\) & \(94.7\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(0.59\) & \(32.07\) & \(32.61\) & \(95.3\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(0.82\) & \(32.00\) & \(32.54\) & \(95.2\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(5.64\) & \(31.25\) & \(32.13\) & \(95.0\)\\
 & 3 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.94\) & \(-1.34\) & \(25.77\) & \(26.10\) & \(95.0\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(-1.01\) & \(27.59\) & \(27.64\) & \(94.9\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(-0.89\) & \(27.50\) & \(27.56\) & \(94.8\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(-0.72\) & \(25.91\) & \(26.36\) & \(95.2\)\\
 & 4 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.93\) & \(-6.87\) & \(30.61\) & \(31.71\) & \(95.1\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.92\) & \(-17.95\) & \(31.47\) & \(32.20\) & \(95.2\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.92\) & \(-16.74\) & \(31.40\) & \(32.13\) & \(95.1\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.93\) & \(-4.80\) & \(31.03\) & \(32.14\) & \(95.3\)\\
\end{tabular}


==> tab/sim-pcate-2-param-1-nocf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.96\) & \(17.90\) & \(52.41\) & \(35.42\) & \(93.4\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.95\) & \(14.58\) & \(47.95\) & \(37.76\) & \(93.7\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.95\) & \(14.37\) & \(48.29\) & \(37.76\) & \(93.6\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.96\) & \(19.67\) & \(48.91\) & \(33.85\) & \(92.7\)\\
 & 2 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.84\) & \(-93.55\) & \(42.97\) & \(40.45\) & \(92.8\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.85\) & \(-86.98\) & \(43.28\) & \(41.24\) & \(93.9\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.85\) & \(-87.28\) & \(43.21\) & \(41.18\) & \(93.8\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.82\) & \(-118.40\) & \(42.18\) & \(38.43\) & \(92.1\)\\
 & 3 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.96\) & \(23.60\) & \(57.77\) & \(36.02\) & \(93.6\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.96\) & \(20.66\) & \(50.58\) & \(38.76\) & \(92.9\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.96\) & \(20.38\) & \(50.79\) & \(38.73\) & \(93.1\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.96\) & \(24.95\) & \(53.82\) & \(34.38\) & \(92.9\)\\
 & 4 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.83\) & \(-102.85\) & \(42.21\) & \(40.37\) & \(94.0\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.83\) & \(-103.79\) & \(42.51\) & \(41.10\) & \(94.6\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.83\) & \(-103.14\) & \(42.43\) & \(41.04\) & \(94.7\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.81\) & \(-129.92\) & \(41.50\) & \(38.52\) & \(93.0\)\\
\(2500\) & 1 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.94\) & \(-1.26\) & \(24.92\) & \(23.81\) & \(93.2\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(-0.15\) & \(26.56\) & \(25.10\) & \(93.3\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(-0.02\) & \(26.50\) & \(25.06\) & \(93.2\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(0.01\) & \(24.63\) & \(23.14\) & \(93.1\)\\
 & 2 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.86\) & \(-73.46\) & \(31.26\) & \(29.00\) & \(92.1\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.87\) & \(-72.11\) & \(31.62\) & \(29.55\) & \(93.4\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.87\) & \(-71.91\) & \(31.57\) & \(29.50\) & \(93.5\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.85\) & \(-91.01\) & \(30.75\) & \(27.85\) & \(91.1\)\\
 & 3 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.93\) & \(-2.87\) & \(24.48\) & \(23.74\) & \(94.3\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.94\) & \(-1.96\) & \(26.28\) & \(25.11\) & \(94.1\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.94\) & \(-1.84\) & \(26.20\) & \(25.04\) & \(94.1\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.94\) & \(-1.18\) & \(24.14\) & \(23.04\) & \(93.4\)\\
 & 4 & \(\hat\beta_{2,\mathrm{oracle}}\) & \(0.86\) & \(-78.88\) & \(30.48\) & \(28.83\) & \(94.2\)\\
 &  & \(\hat\beta_{2,\mathrm{overlap}}\) & \(0.85\) & \(-84.86\) & \(30.95\) & \(29.27\) & \(94.1\)\\
 &  & \(\hat\beta_{2,\mathrm{constant}}\) & \(0.85\) & \(-83.82\) & \(30.89\) & \(29.23\) & \(94.0\)\\
 &  & \(\hat\beta_{2,\mathrm{optimal}}\) & \(0.84\) & \(-97.93\) & \(30.25\) & \(27.93\) & \(93.0\)\\
\end{tabular}


==> tab/sim-pcate-3-param-1-cf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(0.01\) & \(-2.67\) & \(35.10\) & \(30.72\) & \(94.2\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(0.01\) & \(2.80\) & \(38.04\) & \(32.47\) & \(94.3\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(0.01\) & \(2.65\) & \(37.88\) & \(32.40\) & \(94.3\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(0.01\) & \(-0.61\) & \(37.68\) & \(31.57\) & \(94.1\)\\
 & 2 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.06\) & \(-75.58\) & \(38.87\) & \(39.43\) & \(95.2\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.06\) & \(-75.78\) & \(39.83\) & \(39.60\) & \(95.7\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.06\) & \(-75.47\) & \(39.61\) & \(39.53\) & \(95.6\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.06\) & \(-75.39\) & \(39.89\) & \(39.94\) & \(95.6\)\\
 & 3 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(0.00\) & \(-7.72\) & \(41.18\) & \(33.49\) & \(95.6\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(0.01\) & \(-1.20\) & \(47.27\) & \(36.22\) & \(95.8\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(0.01\) & \(-1.23\) & \(46.75\) & \(36.03\) & \(95.6\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(0.01\) & \(-5.53\) & \(47.40\) & \(34.64\) & \(95.6\)\\
 & 4 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.42\) & \(-428.14\) & \(61.92\) & \(43.75\) & \(87.4\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.46\) & \(-474.36\) & \(66.07\) & \(44.46\) & \(84.9\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.46\) & \(-468.94\) & \(65.48\) & \(44.30\) & \(85.1\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.44\) & \(-454.11\) & \(64.98\) & \(45.09\) & \(86.4\)\\
\(2500\) & 1 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.00\) & \(-12.90\) & \(19.67\) & \(20.33\) & \(95.4\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.00\) & \(-12.22\) & \(20.79\) & \(21.48\) & \(95.9\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.00\) & \(-12.35\) & \(20.75\) & \(21.43\) & \(95.7\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.00\) & \(-12.65\) & \(19.83\) & \(20.55\) & \(95.7\)\\
 & 2 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.04\) & \(-51.82\) & \(25.44\) & \(26.72\) & \(96.8\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.04\) & \(-53.10\) & \(25.49\) & \(26.71\) & \(96.2\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.04\) & \(-52.86\) & \(25.46\) & \(26.67\) & \(96.3\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.04\) & \(-50.46\) & \(25.42\) & \(26.54\) & \(96.4\)\\
 & 3 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.01\) & \(-20.80\) & \(20.23\) & \(22.07\) & \(97.2\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.01\) & \(-20.01\) & \(21.47\) & \(23.78\) & \(96.9\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.01\) & \(-19.83\) & \(21.42\) & \(23.66\) & \(97.0\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.01\) & \(-20.83\) & \(20.36\) & \(22.34\) & \(97.2\)\\
 & 4 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.42\) & \(-434.48\) & \(51.92\) & \(29.69\) & \(70.3\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.47\) & \(-483.76\) & \(56.09\) & \(29.93\) & \(64.2\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.47\) & \(-478.22\) & \(55.60\) & \(29.85\) & \(64.7\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.44\) & \(-450.85\) & \(53.43\) & \(30.21\) & \(69.4\)\\
\end{tabular}


==> tab/sim-pcate-3-param-1-nocf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.02\) & \(-29.09\) & \(122.85\) & \(28.06\) & \(92.5\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.03\) & \(-42.86\) & \(154.62\) & \(29.99\) & \(92.3\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.03\) & \(-43.52\) & \(157.16\) & \(30.00\) & \(92.4\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.02\) & \(-30.14\) & \(120.16\) & \(26.78\) & \(91.7\)\\
 & 2 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.06\) & \(-68.64\) & \(35.18\) & \(33.87\) & \(93.4\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.06\) & \(-73.25\) & \(35.48\) & \(34.03\) & \(94.2\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.06\) & \(-72.51\) & \(35.38\) & \(34.00\) & \(94.3\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.06\) & \(-69.08\) & \(34.61\) & \(31.77\) & \(92.6\)\\
 & 3 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.02\) & \(-33.44\) & \(142.10\) & \(30.81\) & \(93.7\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.04\) & \(-52.43\) & \(185.87\) & \(33.68\) & \(93.8\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.04\) & \(-52.80\) & \(188.14\) & \(33.60\) & \(93.8\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.02\) & \(-36.61\) & \(142.71\) & \(29.43\) & \(92.8\)\\
 & 4 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.37\) & \(-382.60\) & \(54.99\) & \(37.84\) & \(84.8\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.42\) & \(-431.26\) & \(58.22\) & \(38.32\) & \(82.0\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.41\) & \(-425.97\) & \(57.81\) & \(38.24\) & \(82.3\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.37\) & \(-384.50\) & \(54.51\) & \(35.93\) & \(81.7\)\\
\(2500\) & 1 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.00\) & \(-13.93\) & \(18.64\) & \(18.30\) & \(94.8\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.00\) & \(-13.27\) & \(19.65\) & \(19.30\) & \(94.8\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.00\) & \(-13.36\) & \(19.61\) & \(19.27\) & \(94.8\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.00\) & \(-13.41\) & \(18.45\) & \(17.75\) & \(94.3\)\\
 & 2 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.04\) & \(-51.38\) & \(24.37\) & \(24.01\) & \(95.3\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.04\) & \(-56.66\) & \(24.57\) & \(24.05\) & \(94.7\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.04\) & \(-56.03\) & \(24.53\) & \(24.03\) & \(94.9\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.04\) & \(-54.78\) & \(24.00\) & \(22.71\) & \(94.1\)\\
 & 3 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.01\) & \(-19.25\) & \(19.36\) & \(19.98\) & \(95.9\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.01\) & \(-18.65\) & \(20.55\) & \(21.49\) & \(95.7\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.01\) & \(-18.48\) & \(20.50\) & \(21.39\) & \(95.6\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.01\) & \(-18.48\) & \(19.05\) & \(19.34\) & \(94.7\)\\
 & 4 & \(\hat\beta_{3,\mathrm{oracle}}\) & \(-0.39\) & \(-401.11\) & \(48.45\) & \(26.83\) & \(67.3\)\\
 &  & \(\hat\beta_{3,\mathrm{overlap}}\) & \(-0.44\) & \(-451.10\) & \(52.64\) & \(27.03\) & \(61.3\)\\
 &  & \(\hat\beta_{3,\mathrm{constant}}\) & \(-0.43\) & \(-445.71\) & \(52.17\) & \(26.98\) & \(61.8\)\\
 &  & \(\hat\beta_{3,\mathrm{optimal}}\) & \(-0.39\) & \(-402.69\) & \(48.33\) & \(25.90\) & \(64.7\)\\
\end{tabular}


==> tab/sim-pcate-4-param-1-cf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.11\) & \(-18.93\) & \(67.05\) & \(61.31\) & \(95.7\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.10\) & \(-25.60\) & \(70.97\) & \(64.73\) & \(95.9\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.10\) & \(-24.83\) & \(70.68\) & \(64.60\) & \(95.8\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.10\) & \(-23.87\) & \(71.00\) & \(62.91\) & \(95.4\)\\
 & 2 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.16\) & \(36.58\) & \(77.90\) & \(78.46\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.16\) & \(36.50\) & \(78.16\) & \(78.99\) & \(95.8\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.16\) & \(37.17\) & \(77.88\) & \(78.81\) & \(95.7\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.16\) & \(38.99\) & \(80.08\) & \(79.64\) & \(95.9\)\\
 & 3 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.10\) & \(-26.49\) & \(77.38\) & \(62.89\) & \(96.5\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.08\) & \(-40.55\) & \(88.12\) & \(67.51\) & \(96.6\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.08\) & \(-39.33\) & \(87.06\) & \(67.22\) & \(96.3\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.09\) & \(-33.24\) & \(88.94\) & \(64.93\) & \(96.5\)\\
 & 4 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.19\) & \(63.88\) & \(77.80\) & \(80.35\) & \(96.5\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.18\) & \(59.73\) & \(78.24\) & \(81.33\) & \(96.6\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.18\) & \(60.38\) & \(77.92\) & \(81.10\) & \(96.6\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.20\) & \(78.34\) & \(80.95\) & \(82.63\) & \(96.6\)\\
\(2500\) & 1 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.13\) & \(5.39\) & \(40.92\) & \(40.77\) & \(94.5\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.13\) & \(5.38\) & \(43.16\) & \(43.03\) & \(95.1\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.13\) & \(5.12\) & \(43.06\) & \(42.95\) & \(95.1\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.13\) & \(4.14\) & \(41.10\) & \(41.19\) & \(94.8\)\\
 & 2 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.14\) & \(18.42\) & \(52.75\) & \(53.58\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.14\) & \(16.63\) & \(53.40\) & \(53.84\) & \(95.2\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.14\) & \(16.58\) & \(53.28\) & \(53.73\) & \(95.0\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.13\) & \(10.40\) & \(52.62\) & \(53.37\) & \(95.3\)\\
 & 3 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.13\) & \(8.37\) & \(40.64\) & \(41.31\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.13\) & \(7.41\) & \(43.09\) & \(44.13\) & \(95.3\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.13\) & \(7.17\) & \(42.95\) & \(43.96\) & \(95.5\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.13\) & \(7.14\) & \(40.84\) & \(41.78\) & \(95.5\)\\
 & 4 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.16\) & \(31.06\) & \(53.66\) & \(54.76\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.14\) & \(19.91\) & \(54.38\) & \(55.05\) & \(94.9\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.15\) & \(20.83\) & \(54.26\) & \(54.92\) & \(95.1\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.16\) & \(40.29\) & \(54.84\) & \(55.62\) & \(95.2\)\\
\end{tabular}


==> tab/sim-pcate-4-param-1-nocf.tex <==

\begin{tabular}{rllrrrrr}
{\(n\)} & {Experiment} & {Estimator} & {Mean} & {Bias} & {RMSE} & {SE} & {Coverage}\\
\(1250\) & 1 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.12\) & \(-6.78\) & \(169.19\) & \(56.09\) & \(94.5\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.14\) & \(18.10\) & \(196.45\) & \(59.84\) & \(94.3\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.14\) & \(19.17\) & \(199.60\) & \(59.87\) & \(94.4\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.12\) & \(-7.30\) & \(161.31\) & \(53.40\) & \(93.4\)\\
 & 2 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.12\) & \(-3.00\) & \(66.85\) & \(67.55\) & \(95.6\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.12\) & \(0.62\) & \(66.78\) & \(68.09\) & \(95.7\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.13\) & \(1.05\) & \(66.66\) & \(68.01\) & \(95.7\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.09\) & \(-34.81\) & \(63.36\) & \(63.46\) & \(95.8\)\\
 & 3 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.11\) & \(-10.26\) & \(191.09\) & \(58.26\) & \(95.3\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.14\) & \(17.91\) & \(227.44\) & \(63.21\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.14\) & \(19.00\) & \(230.11\) & \(63.11\) & \(95.4\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.12\) & \(-9.09\) & \(185.75\) & \(55.43\) & \(94.1\)\\
 & 4 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.15\) & \(23.09\) & \(67.78\) & \(69.81\) & \(95.9\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.15\) & \(21.72\) & \(67.40\) & \(70.46\) & \(96.8\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.15\) & \(22.39\) & \(67.27\) & \(70.34\) & \(96.9\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.12\) & \(-4.11\) & \(64.03\) & \(66.16\) & \(95.5\)\\
\(2500\) & 1 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.12\) & \(-1.27\) & \(38.39\) & \(36.69\) & \(93.7\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.12\) & \(-1.42\) & \(40.54\) & \(38.71\) & \(93.9\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.12\) & \(-1.63\) & \(40.45\) & \(38.64\) & \(93.9\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.12\) & \(-3.39\) & \(37.89\) & \(35.60\) & \(93.1\)\\
 & 2 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.12\) & \(-7.24\) & \(47.82\) & \(48.22\) & \(95.3\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.12\) & \(-5.34\) & \(48.57\) & \(48.56\) & \(94.8\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.12\) & \(-5.50\) & \(48.47\) & \(48.49\) & \(95.0\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.10\) & \(-27.71\) & \(45.82\) & \(45.79\) & \(95.4\)\\
 & 3 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.13\) & \(2.34\) & \(38.19\) & \(37.42\) & \(94.3\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.13\) & \(1.22\) & \(40.61\) & \(39.91\) & \(94.1\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.13\) & \(1.02\) & \(40.48\) & \(39.77\) & \(94.1\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.12\) & \(-1.09\) & \(37.58\) & \(36.22\) & \(93.8\)\\
 & 4 & \(\hat\beta_{4,\mathrm{oracle}}\) & \(0.12\) & \(-5.55\) & \(48.65\) & \(49.54\) & \(95.0\)\\
 &  & \(\hat\beta_{4,\mathrm{overlap}}\) & \(0.11\) & \(-17.45\) & \(49.34\) & \(49.80\) & \(95.0\)\\
 &  & \(\hat\beta_{4,\mathrm{constant}}\) & \(0.11\) & \(-16.23\) & \(49.25\) & \(49.72\) & \(95.0\)\\
 &  & \(\hat\beta_{4,\mathrm{optimal}}\) & \(0.11\) & \(-11.43\) & \(47.19\) & \(47.79\) & \(95.5\)\\
\end{tabular}


==> tab/sim-pcate-param-3-cf-small-sample.tex <==

\begin{tabular}{llrrr}
{Estimator} & {Median} & {Bias} & {MAD} & {SE}\\
\(\hat\beta_{1, \mathrm{oracle}}\) & \(3.00\) & \(6.21\) & \(7.02\) & \(10.72\)\\
\(\hat\beta_{1, \mathrm{overlap}}\) & \(3.00\) & \(6.21\) & \(7.02\) & \(10.72\)\\
\(\hat\beta_{1, \mathrm{constant}}\) & \(3.00\) & \(5.72\) & \(6.98\) & \(10.72\)\\
\(\hat\beta_{1, \mathrm{optimal}}\) & \(3.00\) & \(6.36\) & \(7.08\) & \(10.93\)\\
\(\hat\beta_{2, \mathrm{oracle}}\) & \(0.94\) & \(6.28\) & \(21.71\) & \(31.61\)\\
\(\hat\beta_{2, \mathrm{overlap}}\) & \(0.94\) & \(6.28\) & \(21.71\) & \(31.61\)\\
\(\hat\beta_{2, \mathrm{constant}}\) & \(0.94\) & \(6.32\) & \(21.65\) & \(31.62\)\\
\(\hat\beta_{2, \mathrm{optimal}}\) & \(0.95\) & \(9.93\) & \(21.63\) & \(32.19\)\\
\(\hat\beta_{3, \mathrm{oracle}}\) & \(0.02\) & \(7.62\) & \(16.11\) & \(24.62\)\\
\(\hat\beta_{3, \mathrm{overlap}}\) & \(0.02\) & \(7.62\) & \(16.11\) & \(24.62\)\\
\(\hat\beta_{3, \mathrm{constant}}\) & \(0.02\) & \(7.08\) & \(16.00\) & \(24.63\)\\
\(\hat\beta_{3, \mathrm{optimal}}\) & \(0.01\) & \(1.10\) & \(16.31\) & \(25.11\)\\
\(\hat\beta_{4, \mathrm{oracle}}\) & \(0.12\) & \(-6.57\) & \(32.56\) & \(49.21\)\\
\(\hat\beta_{4, \mathrm{overlap}}\) & \(0.12\) & \(-6.57\) & \(32.56\) & \(49.21\)\\
\(\hat\beta_{4, \mathrm{constant}}\) & \(0.12\) & \(-6.35\) & \(32.57\) & \(49.21\)\\
\(\hat\beta_{4, \mathrm{optimal}}\) & \(0.11\) & \(-14.67\) & \(33.39\) & \(50.20\)\\
\end{tabular}

